Inferring SQL Queries Using Program Synthesis

Developing high-performance applications that interact with databases is a difficult task, as developers need to understand both the details of the language in which their applications are written in, and also the intricacies of the relational model. One popular solution to this problem is the use of object-relational mapping (ORM) libraries that provide transparent access to the database using the same language that the application is written in. Unfortunately, using such frameworks can easily lead to applications with poor performance because developers often end up implementing relational operations in application code, and doing so usually does not take advantage of the optimized implementations of relational operations, efficient query plans, or push down of predicates that database systems provide. In this paper we present QBS, an algorithm that automatically identifies fragments of application logic that can be pushed into SQL queries. The QBS algorithm works by automatically synthesizing invariants and postconditions for the original code fragment. The postconditions and invariants are expressed using a theory of ordered relations that allows us to reason precisely about the contents and order of the records produced even by complex code fragments that compute joins and aggregates. The theory is close in expressiveness to SQL, so the synthesized postconditions can be readily translated to SQL queries. Using 40 code fragments extracted from over 120k lines of open-source code written using the Java Hibernate ORM, we demonstrate that our approach can convert a variety of imperative constructs into relational specifications.

==> commondefs <==
#
# See the manual page for "commondefs" for more information.
#

INCLDIR = $(ROOT)/usr/include
TEXDIR = ../tex-macros

COMMONRULES = $(MAKEDIR)/commonrules

SOURCES = $(CFILES) $(C++FILES) $(YFILES) $(LFILES) $(AFILES)
OBJECTS = $(CFILES:.c=.o) $(C++FILES:.C=.o)
DIRT = *.o core *.aux *.dvi *.log *.stamp *.i *.bbl *.[ib]lg $(LDIRT)
GENERATED = .dependtime Makedepend Makedepend.bak
RM = rm -f
MKDEPFILE = Makedepend
MKDEPEND = makedepend
MKDEPFLAGS = -Y
MKDEPC++FLAGS = $(C++DEFS) $(C++INCS) $(MKDEPFLAGS)
MKDEPCFLAGS = $(CDEFS) $(CINCS) $(MKDEPFLAGS)

.SUFFIXES: .C .ps .i .txt .h
.SUFFIXES: .tex .dvi .ind .idx .bbl .aux .glo .aux .stamp .pdf .eps

GNUBIN = /usr/local

ATTC++ = CC
DECC++ = cxx
GNUC++ = g++

CC = cc
C++ = $(GNUC++)
YACC = bison
DVIPS = dvips

C++F = $(C++) $(C++FLAGS)
CCF = $(CC) $(CFLAGS)

C++FLAGS = $(C++OPTS) $(C++DEFS) $(C++INCS)

C++INCS = $(GC++INCS) $(LC++INCS)
C++OPTS = $(GC++OPTS) $(LC++OPTS)
C++DEFS = $(GC++DEFS) $(LC++DEFS)

GC++OPTS = $(OPTIMIZER)

CFLAGS = $(COPTS) $(CDEFS) $(CINCS)
COPTS = $(GCOPTS) $(LCOPTS)
CDEFS = $(GCDEFS) $(LCDEFS)
CINCS = $(GCINCS) $(LCINCS)

GCOPTS = $(OPTIMIZER)

M3F = $(M3) $(M3FLAGS)
M3 = m3
M3PP = m3pp

LDFLAGS = $(LLDFLAGS) $(GLDFLAGS)
LLDFLAGS = $(LLDLIBS) $(LLDOPTS) 

SEP=:
#SEP=\;         # for MikTeX+Cygwin
TEXINPUTS = .$(SEP)$(TEXDIR)$(SEP)
LATEX = TEXINPUTS="$(TEXINPUTS)" latex --output-directory='$(BUILD)'
PDFLATEX = TEXINPUTS="$(TEXINPUTS)" pdflatex --output-directory='$(BUILD)'

# Directory for TeX's generated files.
BUILD = .
# BUILDD should be equivalent to $(BUILD)/
BUILDD =
VPATH = $(BUILD)


==> commonrules <==
# Some basic recursive rules for building, installing, and cleaning up
# a source tree
#
subdirs:
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make); \
	fi; done;

clean:  localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

localclean:
	$(RM) $(DIRT)

clobber: localclean
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;
	$(RM) $(TARGETS) $(GENERATED)

install: default localinstall
	@sub="$(SUBDIRS)"; \
	for i in $$sub; do if test -n "$$i"; then \
	      (cd $$i; make $@); \
	fi; done;

incdepend: .dependtime
depend: .dependtime

.dependtime: $(SOURCES)
	touch temp
	$(MKDEPEND) $(MKDEPC++FLAGS) -f temp $(C++FILES)
	touch $(MKDEPFILE)
	$(MKDEPEND) $(MKDEPCFLAGS) -f $(MKDEPFILE) $(CFILES)
	cat temp >> $(MKDEPFILE)
	rm -f temp
	touch $@

# Rules for TeX files
#
# The line that runs LATEX needs to run inside a subshell to turn off
# "make"'s status checking. It blows away .aux because the .aux file
# created is bad and also breaks bibtex. It touches .stamp to force a
# rebuild.
.tex.dvi:
	@if test -r "$*.aux"; \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev"; \
	   else echo > "$(BUILDD)$*.auxprev"; \
	fi
	@echo "$(LATEX) $<"
	@sh -c "$(LATEX) $< || (rm -f $*.aux; sleep 1; touch "$(BUILDD)$*.stamp"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev"; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch "$(BUILDD)$*.stamp"; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f "$(BUILDD)$*.auxprev"

.tex.pdf:
	@if test -r "$(BUILDD)$*.aux"; \
	   then cp "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev"; \
	   else echo > "$(BUILDD)$*.auxprev"; \
	fi
	@echo "$(PDFLATEX) $<"
	@sh -c "$(PDFLATEX) $< || (rm -f $*.aux; sleep 1; touch \"$(BUILDD)$*.stamp\"; exit 1)"
	@-cmp -s "$(BUILDD)$*.aux" "$(BUILDD)$*.auxprev"; \
	if test $$? = 1; \
	then \
	    sleep 1; \
	    echo "==> Rebuilding $@"; \
	    touch "$(BUILDD)$*.stamp"; \
	    $(MAKE) $@; \
	else \
	    echo "==> No need to rebuild $@"; \
	fi
	@rm -f "$(BUILDD)$*.auxprev"

# must add dependencies like
#    foo.ind: foo.stamp
#    foo.dvi: foo.ind
# to use this rule properly.
.tex.ind:
	@if [ -f $*.idx ]; then \
	   echo makeindex $*.idx; \
	   makeindex $*.idx; \
	else \
	   echo touch $@; \
	   touch $@; \
        fi

# must add dependencies like
#    foo.bbl: foo.bib
#    foo.dvi: foo.bbl
# to use this rule properly.
.tex.bbl:
	@if [ -r $*.aux ]; then echo bibtex $*; sh -c "bibtex $(BIBOPTS) $* || echo"; else echo; fi

.tex.stamp: # backward compatibility
	touch $@

.dvi.ps:
	$(DVIPS) $(DVIPSOPTS) $< -o $@
.eps.pdf:
	epstopdf $(EPSTOPDFOPTS) $<

#
# Rules for C++ and .i files
#

.C.i:
	$(C++F) -E $< > $@

.c.i:
	$(CCF) -E $< > $@

.C.o:
	$(C++F) -c $<

# include $(M3SU)    # old Modula-3 rules


==> conclusions.tex <==
\section{Conclusions}
\seclabel{conclusions}
In this paper, we presented the \qbs algorithm for inferring 
relational specifications from 
imperative code that retrieves data using ORM libraries. Our algorithm works
by automatically inferring loop invariants and postconditions associated with
the source program, and converting the validated postcondition into SQL queries.
Our approach is both sound and precise in preserving the ordering of records.
In developing the algorithm, we designed a 
new theory of ordered relations that allows efficient encoding
of relational operations into a predicate language. We implemented a prototype 
of the algorithm, and demonstrated the 
applicability and limits using a variety of benchmarks from both real-world applications and 
manually-constructed examples.



==> relatedWork.tex <==
\section{Related Work}
\seclabel{relatedWork}

The idea of inferring relational specifications from imperative code constructs 
was first studied in \cite{wc07, wic08}. The work uses abstract interpretation
and attribute grammar to extract SQL queries
from Java programs. The idea is to compute the set of data access paths that 
a piece of imperative code traverses, and replace the imperative code that performs
the explicit path traversal with SQL queries. The analysis can be applied
to recursive function calls, but does not handle code fragments with loop-carried
dependencies, or fragments that implement join or aggregation. It is unclear
how this method (modeling relational operations as access paths) can be extended 
to handle such cases.

In contrast, our implementation
is able to infer both relational join and aggregation from imperative code. We
currently do not handle recursive function calls, although we have not encountered
the use of recursive functions in the two real-world applications used in our experiments. 

\paragraph{Modeling relational operations}
Our ability to infer relational specifications from imperative code 
relies on using the theory of ordered relations to connect the imperative 
and relational worlds. Previous work modeled such operations differently.
In addition to modeling relational operations using  data access paths, 
other work has modeled relational databases using bags \cite{cooper}, sets \cite{alloy}, and 
nested relational calculus \cite{kleisli}. 
In that respect, one key insight of our work is that ordered relations
are the right abstraction for our purpose, as they are similar to the 
interfaces provided by the ORM libraries in the imperative code, 
and allow us to design a sound and precise transformation
into SQL. Other model choices, such as the theory of sets, would be closer
to the relational model, but would make reasoning about
operations such as \top{} difficult, as elements in a set are not ordered.

To our knowledge, our work is the first one to address the issue of precision, 
i.e., the ordering of records, in relational transformations. 
Precision would not be an
issue if the source program only operated on orderless data structures such 
as sets or did not perform any relational operations that create new records,
such as joins. Unfortunately, most imperative
languages (such as Java) provide interfaces based on ordered data structures,
making this problematic. The benchmarks in our experiments also show that 
implementing joins in imperative code is a relatively common operation. 

\paragraph{Automatic mining of program invariants}
Our verification-based approach to finding a translatable postcondition is
similar to that used in earlier work \cite{jreq, hadoopToSQL}, 
although previous work acknowledges
that finding invariants is difficult and instead
uses a symbolic execution based approach in reasoning about program behavior in 
loops. The idea of 
scanning the source program to generate the synthesis template is inspired by 
the PINS algorithm \cite{sg11}, although in our work we do not require user
intervention. Meanwhile, there has been substantial earlier work on 
automatically detecting loop invariants, such as 
using predicate refinement \cite{fq02} or dynamic approaches like 
the Daikon system \cite{daikon} and invGen \cite{invGen}. There has also been work on
using synthesis 
to discover invariants \cite{sg09}. Our work differs from previous approaches
in that we only need to discover invariants and 
postconditions that are {\it strong enough} 
to validate the transformation, and our predicate grammar and translatable 
expressions greatly prune the space of invariants to those needed for common relational
operations, rather than those needed for general-purpose programs.


\paragraph{Integrated query languages}
Integrating programming languages and database query languages into a single language has been an
active research area, with projects such as LINQ \cite{linq}, Kleisli \cite{kleisli},
Links \cite{links}, JReq \cite{jreq}, the functional language proposed in \cite{cooper},
Ferry \cite{ferry}, and DBPL \cite{dbpl}.
These solutions provide a means to embed database queries in imperative programs without
using ORM-like libraries, or requiring users to embed SQL in their code.
Unfortunately, many of them do not support all relational operations, and 
the syntax of many of such languages are still quite similar to 
SQL, meaning that developers still need to learn new programming concepts.

\paragraph{Improving performance of database programs by code transformation}
There is also work in terms of improving application performance 
by transforming loops and reordering statements 
to expose opportunities for query batching 
\cite{dbBridge, cook2011remote}, and pushing computations into the database to improve
application performance \cite{pyxis}. Our work is orthogonal to this 
line of research. After converting portions of the source code into SQL
queries, such code transformation tools can still be applied to gain 
additional performance improvement.

